Hunting a charged Higgs boson pair in proton-proton collisions

We explore the production and possible detection of a charged scalar Higgs pair $H^-H^+$ decaying into the final state $\mu\nu_{\mu}cb$ in proton-proton collisions at the LHC and its next step, the High Luminosity LHC (HL-LHC). The charged scalars are predicted within the theoretical framework of the Two-Higgs Doublet Model of type III (2HDM-III). As a test and validation of the model, we identify regions of the 2HDM-III parameter space that accommodate the current excess of events at $3\sigma$ in the process $\mathcal{BR}(t\to H^{\pm}b)\times \mathcal{BR}(H^{\pm}\to cb)$ for $M_{H^{\pm}}=130$ GeV, as reported by the ATLAS collaboration. Theoretical and additional experimental constraints are also included. Based on this, we propose realistic scenarios that could be brought under experimental scrutiny at the HL-LHC. Assuming the most favorable scenario, we predict a signal significance at the level of $5\sigma$ for a charged scalar boson mass $M_{H^{\pm}}$ in the $100-350$ GeV range.

==> References.tex <==
\begin{thebibliography}{99}
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	% \bibitem{ref1} footnote 	
		%\cite{ATLAS:2023ofo}
		\bibitem{ATLAS:2023ofo}
		G.~Aad \textit{et al.} [ATLAS],
		%``Search for a new pseudoscalar decaying into a pair of muons in events with a top-quark pair at s=13\,\,TeV with the ATLAS detector,''
		Phys. Rev. D \textbf{108} (2023) no.9, 092007
		doi:10.1103/PhysRevD.108.092007
		[arXiv:2304.14247 [hep-ex]].
		%4 citations counted in INSPIRE as of 15 Feb 2024	
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{ATLAS:2012nhc}
		\bibitem{ATLAS:2012nhc}
		G.~Aad \textit{et al.} [ATLAS],
		%``Search for charged Higgs bosons decaying via $H^{+} \to \tau \nu$ in top quark pair events using $pp$ collision data at $\sqrt{s}=7$ TeV with the ATLAS detector,''
		JHEP \textbf{06} (2012), 039
		doi:10.1007/JHEP06(2012)039
		[arXiv:1204.2760 [hep-ex]].
		%281 citations counted in INSPIRE as of 15 Feb 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
		%\cite{CMS:2012fgz}
		\bibitem{CMS:2012fgz}
		S.~Chatrchyan \textit{et al.} [CMS],
		%``Search for a Light Charged Higgs Boson in Top Quark Decays in $pp$ Collisions at $\sqrt{s}=7$ TeV,''
		JHEP \textbf{07} (2012), 143
		doi:10.1007/JHEP07(2012)143
		[arXiv:1205.5736 [hep-ex]].
		%250 citations counted in INSPIRE as of 15 Feb 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{ATLAS:2023bzb}
		\bibitem{ATLAS:2023bzb}
		G.~Aad \textit{et al.} [ATLAS],
		%``Search for a light charged Higgs boson in $t \rightarrow H^{\pm}b$ decays, with $H^{\pm} \rightarrow cb$, in the lepton+jets final state in proton-proton collisions at $\sqrt{s}=13$ TeV with the ATLAS detector,''
		JHEP \textbf{09} (2023), 004
		doi:10.1007/JHEP09(2023)004
		[arXiv:2302.11739 [hep-ex]].
		%10 citations counted in INSPIRE as of 24 Feb 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Hernandez-Sanchez:2020vax}
		\bibitem{Hernandez-Sanchez:2020vax}
		J.~Hern\'andez-S\'anchez, C.~G.~Honorato, S.~Moretti and S.~Rosado-Navarro,
		%``Charged Higgs boson production via $cb$ -fusion at the Large Hadron Collider,''
		Phys. Rev. D \textbf{102}, no.5, 055008 (2020)
		doi:10.1103/PhysRevD.102.055008
		[arXiv:2003.06263 [hep-ph]].
		%11 citations counted in INSPIRE as of 17 Jul 2023
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
		%\cite{Felix-Beltran:2013tra}
		\bibitem{Felix-Beltran:2013tra} 
		O.~F\'elix-Beltr\'an, F.~Gonz\'alez-Canales, J.~Hern\'andez-S\'anchez, S.~Moretti, R.~Noriega-Papaqui and A.~Rosado,
		%``Analysis of the quark sector in the 2HDM with a four-zero Yukawa texture using the most recent data on the CKM matrix,''
		Phys.\ Lett.\ B {\bf 742}, 347 (2015)
		%%doi:10.1016/j.physletb.2015.02.003
		[arXiv:1311.5210 [hep-ph]].
		%%CITATION = %%doi:10.1016/j.physletb.2015.02.003;%%
		%8 citations counted in INSPIRE as of 15 Sep 2018
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{HernandezSanchez:2012eg}
		\bibitem{HernandezSanchez:2012eg} 
		J.~Hern\'andez-S\'anchez, S.~Moretti, R.~Noriega-Papaqui and A.~Rosado,
		%``Off-diagonal terms in Yukawa textures of the Type-III 2-Higgs doublet model and light charged Higgs boson phenomenology,''
		JHEP {\bf 1307}, 044 (2013)
		%%doi:10.1007/JHEP07(2013)044
		[arXiv:1212.6818 [hep-ph]].
		%%CITATION = %%doi:10.1007/JHEP07(2013)044;%%
		%24 citations counted in INSPIRE as of 15 Sep 2018
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Arroyo-Urena:2020mgg}
		\bibitem{Arroyo-Urena:2020mgg}
		M.~A.~Arroyo-Ure\~na, T.~A.~Valencia-P\'erez, R.~Gait\'an, J.~H.~Montes De Oca and A.~Fern\'andez-T\'ellez,
		%``Flavor-changing decay $h\to \tau\mu$ at super hadron colliders,''
		JHEP \textbf{08} (2020), 170
		doi:10.1007/JHEP08(2020)170
		[arXiv:2002.04120 [hep-ph]].
		%5 citations counted in INSPIRE as of 28 Jan 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		
		%\cite{Arroyo-Urena:2019qhl}
		\bibitem{Arroyo-Urena:2019qhl}
		M.~A.~Arroyo-Ure\~na, R.~Gait\'an, E.~A.~Herrera-Chac\'on, J.~H.~Montes de Oca Y. and T.~A.~Valencia-P\'erez,
		%``Search for the $t\to ch$ decay at hadron colliders,''
		JHEP \textbf{07} (2019), 041
		doi:10.1007/JHEP07(2019)041
		[arXiv:1903.02718 [hep-ph]].
		%11 citations counted in INSPIRE as of 07 May 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		
		%\cite{Arroyo-Urena:2013cyf}
		\bibitem{Arroyo-Urena:2013cyf}
		M.~A.~Arroyo-Ure\~na, J.~L.~Diaz-Cruz, E.~D\'\i{}az and J.~A.~Orduz-Ducuara,
		%``Flavor violating Higgs signals in the Texturized Two-Higgs Doublet Model (THDM-Tx),''
		Chin. Phys. C \textbf{40} (2016) no.12, 123103
		doi:10.1088/1674-1137/40/12/123103
		[arXiv:1306.2343 [hep-ph]].
		%46 citations counted in INSPIRE as of 14 Jul 2022
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
		%\cite{CMS:2017con}
		\bibitem{CMS:2017con}
		A.~M.~Sirunyan \textit{et al.} [CMS],
		%``Search for lepton flavour violating decays of the Higgs boson to $\mu\tau$ and e$\tau$ in proton-proton collisions at $\sqrt{s}=$ 13 TeV,''
		JHEP \textbf{06} (2018), 001
		doi:10.1007/JHEP06(2018)001
		[arXiv:1712.07173 [hep-ex]].
		%105 citations counted in INSPIRE as of 28 Jan 2024		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{ATLAS:2019pmk}
		\bibitem{ATLAS:2019pmk}
		G.~Aad \textit{et al.} [ATLAS],
		%``Searches for lepton-flavour-violating decays of the Higgs boson in $\sqrt{s}=13$ TeV pp collisions with the ATLAS detector,''
		Phys. Lett. B \textbf{800} (2020), 135069
		doi:10.1016/j.physletb.2019.135069
		[arXiv:1907.06131 [hep-ex]].
		%80 citations counted in INSPIRE as of 28 Jan 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{CMS:2022mgd}
		\bibitem{CMS:2022mgd}
		A.~Tumasyan \textit{et al.} [CMS],
		%``Measurement of the B$^0_\mathrm{S}$$\to$$\mu^+\mu^-$ decay properties and search for the B$^0$$\to$$\mu^+\mu^-$ decay in proton-proton collisions at $\sqrt{s}$ = 13 TeV,''
		Phys. Lett. B \textbf{842} (2023), 137955
		doi:10.1016/j.physletb.2023.137955
		[arXiv:2212.10311 [hep-ex]].
		%67 citations counted in INSPIRE as of 10 Apr 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		
		%\cite{Workman:2022ynf}
		\bibitem{Workman:2022ynf}
		R.~L.~Workman \textit{et al.} [Particle Data Group],
		%``Review of Particle Physics,''
		PTEP \textbf{2022}, 083C01 (2022)
		doi:10.1093/ptep/ptac097
		%3 citations counted in INSPIRE as of 12 Jul 2022
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Muong-2:2021ojo}
		\bibitem{Muong-2:2021ojo}
		B.~Abi \textit{et al.} [Muon g-2],
		%``Measurement of the Positive Muon Anomalous Magnetic Moment to 0.46 ppm,''
		Phys. Rev. Lett. \textbf{126} (2021) no.14, 141801
		doi:10.1103/PhysRevLett.126.141801
		[arXiv:2104.03281 [hep-ex]].
		%1594 citations counted in INSPIRE as of 28 Jan 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{ATLAS:2021ifb}
		\bibitem{ATLAS:2021ifb}
		G.~Aad \textit{et al.} [ATLAS],
		%``Search for Higgs boson pair production in the two bottom quarks plus two photons final state in $pp$ collisions at $\sqrt{s}=13$ TeV with the ATLAS detector,''
		Phys. Rev. D \textbf{106} (2022) no.5, 052001
		doi:10.1103/PhysRevD.106.052001
		[arXiv:2112.11876 [hep-ex]].
		%99 citations counted in INSPIRE as of 11 Apr 2024	
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bibitem{ATLAS-CONF}
		ATLAS Collaboration, CERN Report No. ATLAS-CONF-2017-055, 2017.
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bibitem{Sirunyan:2018zut} 
		A.~M.~Sirunyan {\it et al.} [CMS Collaboration],
		%``Search for additional neutral MSSM Higgs bosons in the $\tau\tau$ final state in proton-proton collisions at $\sqrt{s}=$ 13 TeV,''
		JHEP {\bf 1809}, 007 (2018)
		doi:10.1007/JHEP09(2018)007
		[arXiv:1803.06553 [hep-ex]].
		%%CITATION = doi:10.1007/JHEP09(2018)007;%%
		%83 citations counted in INSPIRE as of 06 Jan 2020
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{ATLAS:2018gfm}
		\bibitem{ATLAS:2018gfm}
		M.~Aaboud \textit{et al.} [ATLAS],
		%``Search for charged Higgs bosons decaying via $H^{\pm} \to \tau^{\pm}\nu_{\tau}$ in the $\tau$+jets and $\tau$+lepton final states with 36 fb$^{-1}$ of $pp$ collision data recorded at $\sqrt{s} = 13$ TeV with the ATLAS experiment,''
		JHEP \textbf{09} (2018), 139
		doi:10.1007/JHEP09(2018)139
		[arXiv:1807.07915 [hep-ex]].
		%208 citations counted in INSPIRE as of 28 Mar 2024		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bibitem{Ciuchini:1997xe} 
		M.~Ciuchini, G.~Degrassi, P.~Gambino and G.~F.~Giudice,
		%``Next-to-leading QCD corrections to $B \to  X_s \gamma$: Standard Model and two Higgs doublet model,''
		Nucl.\ Phys.\ B {\bf 527}, 21 (1998)
		doi:10.1016/S0550-3213(98)00244-2
		[hep-ph/9710335].
		%%CITATION = doi:10.1016/S0550-3213(98)00244-2;%%
		%434 citations counted in INSPIRE as of 24 Jan 2020
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Misiak:2017bgg}
		\bibitem{Misiak:2017bgg} 
		M.~Misiak and M.~Steinhauser,
		%``Weak radiative decays of the B meson and bounds on $M_{H^\pm }$ in the Two-Higgs-Doublet Model,''
		Eur.\ Phys.\ J.\ C {\bf 77}, no. 3, 201 (2017)
		doi:10.1140/epjc/s10052-017-4776-y
		[arXiv:1702.04571 [hep-ph]].
		%%CITATION = doi:10.1140/epjc/s10052-017-4776-y;%%
		%138 citations counted in INSPIRE as of 24 Jan 2020
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%\cite{Beneke:2019slt}
		\bibitem{Beneke:2019slt}
		M.~Beneke, C.~Bobeth and R.~Szafron,
		%``Power-enhanced leading-logarithmic QED corrections to $B_q \to \mu^+\mu^-$,''
		JHEP \textbf{10} (2019), 232
		[erratum: JHEP \textbf{11} (2022), 099]
		doi:10.1007/JHEP10(2019)232
		[arXiv:1908.07011 [hep-ph]].
		%154 citations counted in INSPIRE as of 10 Apr 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Buras:2012ru}
		\bibitem{Buras:2012ru}
		A.~J.~Buras, J.~Girrbach, D.~Guadagnoli and G.~Isidori,
		%``On the Standard Model prediction for BR(B{s,d} to mu+ mu-),''
		Eur. Phys. J. C \textbf{72} (2012), 2172
		doi:10.1140/epjc/s10052-012-2172-1
		[arXiv:1208.0934 [hep-ph]].
		%271 citations counted in INSPIRE as of 10 Apr 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Inami:1980fz}
		\bibitem{Inami:1980fz}
		T.~Inami and C.~S.~Lim,
		%``Effects of Superheavy Quarks and Leptons in Low-Energy Weak Processes k(L) ---\ensuremath{>} mu anti-mu, K+ ---\ensuremath{>} pi+ Neutrino anti-neutrino and K0 \ensuremath{<}---\ensuremath{>} anti-K0,''
		Prog. Theor. Phys. \textbf{65} (1981), 297
		[erratum: Prog. Theor. Phys. \textbf{65} (1981), 1772]
		doi:10.1143/PTP.65.297
		%1871 citations counted in INSPIRE as of 10 Apr 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Harnik:2012pb}
		\bibitem{Harnik:2012pb}
		R.~Harnik, J.~Kopp and J.~Zupan,
		%``Flavor Violating Higgs Decays,''
		JHEP \textbf{03} (2013), 026
		doi:10.1007/JHEP03(2013)026
		[arXiv:1209.1397 [hep-ph]].
		%363 citations counted in INSPIRE as of 10 Mar 2023
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Blankenburg:2012ex}
		\bibitem{Blankenburg:2012ex}
		G.~Blankenburg, J.~Ellis and G.~Isidori,
		%``Flavour-Changing Decays of a 125 GeV Higgs-like Particle,''
		Phys. Lett. B \textbf{712} (2012), 386-390
		doi:10.1016/j.physletb.2012.05.007
		[arXiv:1202.5704 [hep-ph]].
		%213 citations counted in INSPIRE as of 10 Mar 2023
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
		%\cite{Arroyo-Urena:2020qup}
		\bibitem{Arroyo-Urena:2020qup}
		M.~A.~Arroyo-Ure\~na, R.~Gait\'an and T.~A.~Valencia-P\'erez,
		%``SpaceMath version 1.0 A Mathematica package for beyond the Standard Model parameter space searches,''
		Rev. Mex. Fis. E \textbf{19} (2022) no.2, 020206
		doi:10.31349/RevMexFisE.19.020206
		[arXiv:2008.00564 [hep-ph]].
		%6 citations counted in INSPIRE as of 20 Jul 2022
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%		
		%\cite{Alloul:2013bka}
		\bibitem{Alloul:2013bka}
		A.~Alloul, N.~D.~Christensen, C.~Degrande, C.~Duhr and B.~Fuks,
		%``FeynRules  2.0 - A complete toolbox for tree-level phenomenology,''
		Comput. Phys. Commun. \textbf{185} (2014), 2250-2300
		doi:10.1016/j.cpc.2014.04.012
		[arXiv:1310.1921 [hep-ph]].
		%2400 citations counted in INSPIRE as of 18 Apr 2024		
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bibitem{MadGraphNLO}
		J. Alwall, M. Herquet, F. Maltoni, O. Mattelaer, and T.Stelzer, J. High Energy Phys. 06 (2011) 128.
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Sjostrand:2008vc}
		\bibitem{Sjostrand:2008vc} 
		T.~Sjostrand,
		%``PYTHIA 8 Status Report,''
		doi:10.3204/DESY-PROC-2009-02/41
		arXiv:0809.0303 [hep-ph].
		%%CITATION = doi:10.3204/DESY-PROC-2009-02/41;%%
		%36 citations counted in INSPIRE as of 28 Oct 2019
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		\bibitem{delphes}
		J. de Favereau, C. Delaere, P. Demin, A. Giammanco, V.
		Lemaitre, A. Mertens, and M. Selvaggi, J. High Energy
		Phys. 02 (2014) 057.
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Cacciari:2011ma}
		\bibitem{Cacciari:2011ma}
		M.~Cacciari, G.~P.~Salam and G.~Soyez,
		%``FastJet User Manual,''
		Eur. Phys. J. C \textbf{72} (2012), 1896
		doi:10.1140/epjc/s10052-012-1896-2
		[arXiv:1111.6097 [hep-ph]].
		%5869 citations counted in INSPIRE as of 02 May 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Cacciari:2008gp}
		\bibitem{Cacciari:2008gp}
		M.~Cacciari, G.~P.~Salam and G.~Soyez,
		%``The anti-$k_t$ jet clustering algorithm,''
		JHEP \textbf{04} (2008), 063
		doi:10.1088/1126-6708/2008/04/063
		[arXiv:0802.1189 [hep-ph]].
		%10084 citations counted in INSPIRE as of 02 May 2024
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
		%\cite{Conte:2012fm}
		\bibitem{Woodruff2018}
		K.~Woodruff,
		%``BDT Tutorial,''
		GitHub repository (2018),
		\url{https://github.com/k-woodruff/bdt-tutorial}
		\bibitem{Conte:2012fm}
		E.~Conte, B.~Fuks and G.~Serret,
		%``MadAnalysis 5, A User-Friendly Framework for Collider Phenomenology,''
		Comput. Phys. Commun. \textbf{184} (2013), 222-256
		doi:10.1016/j.cpc.2012.09.009
		[arXiv:1206.1599 [hep-ph]].
		%602 citations counted in INSPIRE as of 30 Apr 2024		
		
		
	\end{thebibliography}
